Robust Optimization as Data Augmentation for Large-scale Graphs

Data augmentation helps neural networks generalize better by enlarging the training set, but it remains an open question how to effectively augment graph data to enhance the performance of GNNs (Graph Neural Networks). While most existing graph regularizers focus on manipulating graph topological structures by adding/removing edges, we offer a method to augment node features for better performance. We propose FLAG (Free Large-scale Adversarial Augmentation on Graphs), which iteratively augments node features with gradient-based adversarial perturbations during training. By making the model invariant to small fluctuations in input data, our method helps models generalize to out-of-distribution samples and boosts model performance at test time. FLAG is a general-purpose approach for graph data, which universally works in node classification, link prediction, and graph classification tasks. FLAG is also highly flexible and scalable, and is deployable with arbitrary GNN backbones and large-scale datasets. We demonstrate the efficacy and stability of our method through extensive experiments and ablation studies. We also provide intuitive observations for a deeper understanding of our method.

==> sections/2-related.tex <==
\section{Related Work}

% We briefly summarize graph neural networks and graph regularizers in line with our topic.

% \textbf{Graph Neural Networks.} There has been a surge of graph learning research in recent years. Graph Neural Networks (GNNs) have been proven to be important tools in analyzing and understanding complex and interactive graph systems in non-Euclidean spaces. One important task for the graph community is to do semi-supervised node classification, aka transductive node classification, on which a series of successful GNN architectures are proposed \citep{defferrard2016convolutional,kipf2016semi,velivckovic2017graph,hamilton2017inductive}. Besides that GNNs have shown their power in solving graph classification and link prediction tasks \citep{xu2018how,zhang2018link}. Generally speaking, GNNs follow the message-passing pipeline to aggregate information from the neighborhood. A formal formulation of message-passing GNNs can be found in Section \ref{pre}. Meanwhile, with the growing size of graph datasets, scalability has been a great issue for graph learning. The aforementioned GNN architectures do full-batch forward pass by default, which is no longer feasible when encountering large-scale datasets. To combat the obstacle, a number of graph batching methods \citep{hamilton2017inductive,chiang2019cluster,zeng2019graphsaint} were proposed to help.

% \textbf{Adversarial Training.}

% Existing graph regularizers mainly focus on augmenting graph structures by modifying edges \citep{rong2019dropedge,hamilton2017inductive,chen2018fastgcn}. We propose to effectively augment graph data using adversarial perturbations. On large-scale image classification tasks, \citet{xie2020adversarial} leveraged adversarial perturbations, along with new batch norm methods, to augment data. \citet{zhu2019freelb,jiang2019smart} added adversarial perturbations in the embedding space and generalized language models further in the fine-tuning phase. \citet{gan2020large} showed that VQA model accuracy was further improved by adversarial augmentation. 

% To clarify, FLAG is intrinsically different from the previous graph adversarial training methods \citep{feng2019graph,deng2019batch,jin2019latent}. \citet{feng2019graph} proposed to reinforce local smoothness to make embeddings within communities similar. All three methods assigned pseudo-labels to test nodes during training time and utilized virtual adversarial training \citep{miyato2018virtual} to make test node predictions similar to their pseudo-labels.  This makes them workable for semi-supervised settings, but not for inductive tasks. Besides the original classification loss term, they all introduced KL loss into the final objective functions, which would at least double the GPU memory usage and make training less efficient and less scalable. In contrast, FLAG requires minimal extra space overhead and can directly work in the original training setup.

% \textbf{GNN Augmentations.} Overfitting is a serious issue for various kinds of neural nets. Generally speaking, GNN augmentations mostly focus on manipulating graph topological structures to mitigate overfitting. On the graph classification task, \citet{gilmer2017neural} proposed virtual nodes, which connect to all original nodes in the graph to improve accuracy. Neighbor Sampling \citep{hamilton2017inductive} randomly samples neighbors for each node when aggregating information to enlarge diversity. \citet{rong2019dropedge} proposed DropEdge, which randomly drops edges from the graph to combat overfitting and oversmoothing. GraphCL \citep{you2020graph} highlighted the importance of structure-based augmentation in the context of contrastive learning.  Finally, \citet{wang2020nodeaug} proposed an attribute replacement scheme for node classification, which swaps uninformative attributes of the central node with other relevant ones on small datasets. 

Existing graph regularizers mainly focus on augmenting graph structures by modifying edges \citep{rong2019dropedge,hamilton2017inductive,chen2018fastgcn}. GraphAT \citep{feng2019graph}, BVAT \citep{deng2019batch}, and LAT \citep{jin2019latent} are three \textit{semi-supervised} methods for training without labels on the node classification task. GraphAT promotes local smoothness by reinforcing the similarity between the predictions of perturbed nodes and their neighbors. BVAT proposed two graph VAT schemes to enhance the output smoothness of GCN; LAT virtually perturbed the first-layer embedding of a GCN classifier to improve its robustness. Although these works involved manipulating the input node features, their methods were semi-supervised VAT pipelines which required complex and specific objective functions, rather than general-purpose data augmentation methods which should be flexible to work with arbitrary objectives. The usage scenario of these methods is also limited to node classification, while data augmentation should function regardless of tasks. Besides those, the formulation of VAT \citep{miyato2018virtual} utilized by these works involves both supervised clean and adversarial robust losses simultaneously. This in practice will require at least twice the GPU memory as the baseline, making them not scalable to large-scale datasets. Overall, no work so far has considered general-purpose feature-based data augmentations for large-scale graphs.


==> tables/free.tex <==
\begin{table}[h]
    
        \centering
        \begin{tabular}{lc}
            \Xhline{2\arrayrulewidth}
            & \texttt{ogbn-products} \\
            Backbone	& Test Acc  \\
            \hline\hline
            GAT  & 79.45\textcolor{gray}{\footnotesize{$\pm$0.59}} \\
            +FLAG$^\diamond$ & \bftab80.64\textcolor{gray}{\footnotesize{$\pm$0.74}} \\
            \hline
            +FLAG$^\dagger$ & 81.29\textcolor{gray}{\footnotesize{$\pm$0.39}} \\
            +FLAG$^\ddagger$ & \bftab81.76\textcolor{gray}{\footnotesize{$\pm$0.45}} \\
            \Xhline{2\arrayrulewidth}
        \end{tabular}
        \caption{Test performance on \texttt{ogbn-products} with GAT as baseline. $\diamond$ denotes model trained in $N/M$ epochs; $\dagger$ denotes $\alpha_u=\alpha_l$; $\ddagger$ denotes $\alpha_u=2\alpha_l$.}
        % \vspace{-8mm}
\end{table}
